Introspective Experience Replay: Look Back When Surprised

In reinforcement learning (RL), experience replay-based sampling techniques play a crucial role in promoting convergence by eliminating spurious correlations. However, widely used methods such as uniform experience replay (UER) and prioritized experience replay (PER) have been shown to have sub-optimal convergence and high seed sensitivity respectively. To address these issues, we propose a novel approach called IntrospectiveExperience Replay (IER) that selectively samples batches of data points prior to surprising events. Our method builds upon the theoretically sound reverse experience replay (RER) technique, which has been shown to reduce bias in the output of Q-learning-type algorithms with linear function approximation. However, this approach is not always practical or reliable when using neural function approximation. Through empirical evaluations, we demonstrate that IER with neural function approximation yields reliable and superior performance compared toUER, PER, and hindsight experience replay (HER) across most tasks.

==> ICML_ IER/icml23/abstract.tex <==
\begin{abstract}

% Experience replay-based sampling techniques are essential to several reinforcement learning (RL) algorithms since they aid in convergence by breaking spurious correlations. The most popular techniques, such as uniform experience replay (\nameu) and prioritized experience replay (\namep), seem to suffer from sub-optimal convergence, and non-robust (highly seed sensitive), respectively. To alleviate this, we introduce a new experience replay method for reinforcement learning, called Introspective Experience Replay (\namel). \namel~picks batches corresponding to data points consecutively before the `surprising' points. Our proposed approach is based on the theoretically rigorous reverse experience replay (\namelo), which can be shown to remove the bias in the error produced by Q-learning type algorithms in the linear approximation setting. However, this can be ineffective and unreliable with neural approximation. We show empirically that \namel~ with neural function approximation learns reliably and has a superior performance compared to the state-of-the-art techniques like uniform experience replay (\nameu), prioritized experience replay (\namep), and hindsight experience replay (\nameh) on the majority of tasks.

In reinforcement learning (RL), experience replay-based sampling techniques play a crucial role in promoting convergence by eliminating spurious correlations. However, widely used methods such as uniform experience replay (\nameu) and prioritized experience replay (\namep) have been shown to have sub-optimal convergence and high seed sensitivity respectively. To address these issues, we propose a novel approach called Introspective Experience Replay (\namel) that selectively samples batches of data points prior to surprising events. Our method builds upon the theoretically sound reverse experience replay (\namelo) technique, which has been shown to reduce bias in the output of Q-learning-type algorithms with linear function approximation. However, this approach is not always practical or reliable when using neural function approximation. Through empirical evaluations, we demonstrate that \namel~with neural function approximation yields reliable and superior performance compared to \nameu, \namep, and hindsight experience replay (\nameh) across most tasks.

\end{abstract}

==> ICML_ IER/icml23/background.tex <==

\section{Background and Proposed Methodology}
\label{prelim}
%\subsection{Reinforcement Learning}
We consider episodic reinforcement learning \citep{sutton2018reinforcement}, where at each time step an agent takes actions $a_t$ in an uncertain environment with state $s_t$, and receives a reward $r_t$. The environment then evolves into a new state $s_{t+1}$ whose law depends only on $s_t,a_t$. Our goal is to (approximately) find the policy $\pi^{*}$ which maps the environmental state $s$ to an action $a$ such that when the agent takes the action $a_t = \pi^{*}(s_t)$, the discounted reward $\mathbb{E}\left[\sum_{t=0}^{\infty}\gamma^{t}r_t\right]$ is maximized. To achieve this, we consider algorithms like DQN (\cite{mnih2015human}), DDPG (\cite{lillicrap2015continuous}) and TD3 (\cite{fujimoto2018addressing}), which routinely use experience replay buffers. In this paper, we introduce a new experience replay method, \namel, and investigate the performance of the aforementioned RL algorithms with this modification. In this work, when we say ``return'', we mean discounted episodic reward. 
% We use the term ``per-step reward'' to denote the reward received at each time step.

%\rk{per-step reward vs reward (episodic). when we say reward, we implicitly mean episodic reward.}
% More specifically, we seek to investigate the following questions:
% \dn{the itemize below seems redundant since we have described most of this in the intro only}
% \begin{itemize}
%     \item \textbf{Does our algorithm help in the convergence towards a better policy?} The performance of most RL algorithms are highly dependent on the type of Replay Buffer algorithm used. We aim to emplore if \namel~learns a superior policy compared to those obtained from other baselines. 
    
%     \item \textbf{Does our algorithm lead to any speedup in convergence?} Reinforcement learning algorithms, in general, are very slow to learn and could take days and millions of steps to converge to a locally optimal policy. We aim to study whether the inclusion of \namel~helps speed up the convergence of these algorithms.
    
%     \item \textbf{Is our algorithm robust across environments?} To efficiently support the practical gains from our algorithm, we aim to show that our proposed methodology not only outperforms other baselines but is consistently doing so across various environments with limited hyperparameter tuning.
    
%     \item \textbf{What influences the performance of our proposed methodology?} We aim to study why our proposed approach does well across different environments. To answer this question, we perform an ablation study between \nameo, \namelo~and \namel~for the reasons highlighted in Section~\ref{understanding_rer}. We also perform an ablation study with FER++ where data points form buffers by processing the forward order from the pivots instead of the reverse order.
    
% \end{itemize}


%\subsection{Deep Q Networks (DQN)}

%\subsection{TD3}
%\section{Traditional RER Method}
\begin{algorithm*}
\caption{Our proposed Introspective Experience Replay (\namel) for Reinforcement Learning}\label{alg:rev_plus}
 \KwIn{Data collection mechanism $\mathbb{T}$, Data buffer $\mathcal{H}$, Batch size $B$, grad steps per Epoch $G$, number of episodes $N$, Importance function $I$, learning procedure $\mathbb{A}$, Uniform Mixing fraction $p$}
 $n \leftarrow 0$\;
 
 \While{$n < N$}
 { $n \leftarrow n+1$\;

  $\mathcal{H} \leftarrow \mathbb{T}(\mathcal{H})$ \hspace*{\fill} \tcp*{\footnotesize Add a new episode to the buffer}

$\mathcal{I} \leftarrow I(\mathcal{H})$ \hspace*{\fill} \tcp*{\footnotesize Compute importance of each data point in the buffer} 

 $P \leftarrow \mathsf{Top}(\mathcal{I};G)$ \hspace*{\fill} \tcp*{\footnotesize Obtain index of top $G$ elements of $\mathcal{I}$} 
 $g \leftarrow 0$\;

 \While{$g< G$}{
 \eIf{$g<(1-p)G$}{
 $D \leftarrow \mathcal{H}[P[g]-B,P[g]]$ \hspace*{\fill} \tcp*{\footnotesize Load batch of previous $B$ examples from pivot $P[g]$} 
 }{
 $D \leftarrow \mathcal{H}[\mathsf{Uniform}(\mathcal{H}, B)]$ \hspace*{\fill} \tcp*{\footnotesize Randomly chose $B$ indices from buffer} 
 }
 $g\leftarrow g+1$\;

 $\mathbb{A}(D)$\hspace*{\fill} \tcp*{\footnotesize Run the learning algorithm with batch data $D$} 
 }
 }
\end{algorithm*}

\subsection{Methodology}
\label{method}
We now describe our main method in a general way where we assume that we have access to a data collection mechanism $\mathbb{T}$ which samples new data points. This then appends the sampled data points to a buffer $\mathcal{H}$ and discards some older data points. The goal is to run an iterative learning algorithm $\mathbb{A}$, which learns from batched data of batch size $B$ in every iteration. We also consider an important metric $I$ associated with the problem. At each step, the data collection mechanism $\mathbb{T}$ collects a new episode and appends it to the buffer $\mathcal{H}$ and discards some old data points, giving us the new buffer as $\mathcal{H} \leftarrow \mathbb{T}(\mathcal{H})$. We then sort the entries of $\mathcal{H}$ based on the importance metric $I$ and store the indices of the top $G$ data points in an array $P = [P[0],\dots,P[G-1]]$. Then for every index in $P$, we run the learning algorithm $\mathbb{A}$ with the batch $D = (\mathcal{H}(P[i]),\dots,\mathcal{H}(P[i]-B+1))$. In some cases, we can `mix'\footnote{Mixing here denotes sampling with a given probability from one sampler A, and filling the remaining samples of a batch with sampler B.} this with the standard \nameu~sampling mechanism to reduce bias of the stochastic gradients with respect to the empirical distribution in the buffer, as shown below. Our experiments show that this amalgamation helps convergence in certain cases. We describe this procedure in Algorithm~\ref{alg:rev_plus}. 

%\paragraph{Can we infuse \namel~with \nameh?}

%In practice, the two methodologies follow very different intuitions. The \namel~samples differ from \nameu, whereas \nameh~adds episodes differently from \nameu. Since the two concepts are disjoint, it is possible to infuse the two concepts together, something we call \namek.

In the reinforcement learning setting, $\mathbb{T}$ runs an environment episode with the current policy and appends the transitions and corresponding rewards to the buffer $\mathcal{H}$ in the FIFO order, maintaining a total of $1E6$ data points, usually. We choose $\mathbb{A}$ to be an RL algorithm like TD3 or DQN or DDPG. The importance function $I$ is the magnitude of the TD error with respect to the current Q-value estimate provided by the algorithm $\mathbb{A}$ (i.e., $I = |Q(s,a) - R(s,a) - \gamma \sup_{a^{\prime}}Q^{\mathsf{target}}(s^{\prime},a^{\prime})|$). When the data collection mechanism ($\mathbb{T}$) is the same as in \nameu, we will call this method \textbf{\namel}. In optimistic experience replay (\nameo), we take $\mathbb{T}$ to be the same as in \nameu. However, we query top $BG$ data points from the buffer $\mathcal{H}$ and return $G$ disjoint batches each of size $B$ from these `important' points. It is clear that \namel~is a combination of \nameo~and \namelo. Notice that we can also consider the data collection mechanism like that of \nameh, where examples are labeled with different goals, i.e. $\mathbb{T}$ has now been made different, keeping the sampling process exactly same as before. In this case, we will call our algorithm \textbf{\namek}. Our experiment in Enduro and Acrobat depicts an example of this successful coalition. We also consider the \namelo~method, which served as a motivation for our proposed approach. Under this sampling methodology, the batches are drawn from $\mathcal{H}$ in the temporally reverse direction. This approach is explored in the works mentioned in Section~\ref{sec:rev_sweep}. We discuss this methodology in more detail in Appendix~\ref{rer}. 

\subsection{Didactic Toy Example}
\label{sec:toy_example}
In this section, we discuss the working of \namel~on a simple environment such as GridWorld-1D, and compare this with some of our baselines such as \nameu, \nameo, \namelo, and IER (F). In this environment, the agent lives on a discrete 1-dimensional grid of size 40 with a max-timestep of 1000 steps, and at each time step, the agent can either move left or right by one step. The agent starts from the \textit{starting state} (S; $[6]$), the goal of the agent is to reach \textit{goal state} (G; $[40]$) getting a reward of $+1$, and there is also a \textit{trap state} (T; $[3]$), where the agents gets a reward of $-2$. The reward in every other state is $0$. For simplicity, we execute an offline exploratory policy where the agent moves left or right with a probability of half and obtain a buffer of size 30000. The rewarding states occur very rarely in the buffer since it is hard to reach for this exploration policy. The episode ends upon meeting either of two conditions: (i) the agent reaches the terminal state, which is the \textit{goal state}, or (ii) the agent has exhausted the max-timestep condition and has not succeeded in reaching any terminal state. An overview of our toy environment is depicted in Figure~\ref{fig:gridworld_env}. Other hyperparameters crucial to replicating this experiment are described in Appendix~\ref{appendix-hyperparam}.

In this example, reaching the goal state as quickly as possible is vital to receive a positive reward and avoid the fail state. Therefore, it is essential to understand the paths which reach the goal state.
Figure~\ref{fig:gridworld_count} depicts the number of times each state occurs in the buffer. Furthermore, the remaining subplots of Figure~\ref{fig:gridworld_v_function} depict the \textit{Absolute Frequency} of our off-policy algorithm trained in this environment. A state's ``absolute frequency'' is the number of times the replay technique samples a given state during the algorithm's run. The experiments on this simple didactic toy environment do highlight a few interesting properties: \newline
\textbf{Comparison of \nameu~and \namel:} Since the goal state appears very rarely in buffer, \nameu~and \namelo~rarely sample the goal state and hence do not manage to learn effectively. While \namelo~naturally propagates the information about the reward back in time to the states that led to the reward, it does not often sample the rewarding state. \newline
\textbf{Limitation of \nameo:}  While \nameo~samples a lot from the states close to the goal state, the information about the reward does not propagate to the start state. We refer to the bottleneck in Figure~\ref{fig3} where some intermediate states are not sampled. \newline%This leads to bias in \nameo. (see Figure~\ref{fig3})    
\textbf{Advantage of \namel:} \namel~prioritizes sampling from the goal state and propagates the reward backward so that the entire path leading to the reward is now aware of how to reach the reward. Therefore, a combination of \namelo~and \nameo~reduces the sampling bias in \nameo~by preventing the bottlenecks seen in Figure~\ref{fig3}. \newline 
\textbf{Bottleneck of IER (F):} 
IER (F) has a more significant bottleneck when compared to \namelo~and chooses to sample the non-rewarding middle states most often. Also, note that whenever IER (F) chooses the goal state as the pivot, it selects the rest of the batch to overflow into the next episode, which begins at the starting state. This does not allow the algorithm to effectively learn the path which \emph{led} to the goal state. 
%     \begin{enumerate}
% %Therefore, the agent knows the direction to travel from the start state. This reduces the bias in \nameo, which created bottlenecks that prevented 
%     %\item It is not clear from this When FER++ encounters the goal state as the surprising state, it picks the buffer which spills over into the next episode and hence does not reliabl
    

% \end{enumerate}

\begin{figure*}[hbt!]
\centering
\subfigure[GridWorld-1D environment]{%
\label{fig:gridworld_env}
\includegraphics[width=0.33\linewidth]{figures/didactic_toy_example/gridworld_env.pdf}}
\quad
\subfigure[Buffer]{%
\label{fig:gridworld_count}
\includegraphics[width=0.22\linewidth]{figures/didactic_toy_example/gridworld_count.pdf}}
\quad
\subfigure[UER]{%
\label{fig1}
\includegraphics[width=0.22\linewidth]{figures/didactic_toy_example/gridworld_uer.pdf}}

\subfigure[RER]{%
\label{fig2}
\includegraphics[width=0.22\linewidth]{figures/didactic_toy_example/gridworld_rer.pdf}}
\quad
\subfigure[OER]{%
\label{fig3}
\includegraphics[width=0.22\linewidth]{figures/didactic_toy_example/gridworld_oer.pdf}}
\quad
\subfigure[IER]{%
\label{fig4}
\includegraphics[width=0.22\linewidth]{figures/didactic_toy_example/gridworld_rer++.pdf}}
\quad
\subfigure[IER (F)]{%
\label{fig5}
\includegraphics[width=0.22\linewidth]{figures/didactic_toy_example/gridworld_fer++.pdf}}
%
\caption{Gridworld-1D environment is depicted in Figure~\ref{fig:gridworld_env}. Distribution of states in the buffer (Figure~\ref{fig:gridworld_count}) and relative frequency of different experience replay samplers on the didactic example of GridWorld-1D environment (Figure~\ref{fig1};\ref{fig2};\ref{fig3};\ref{fig4};\ref{fig5}).}
\label{fig:gridworld_v_function}
\end{figure*}


% In addition to the above example, we also present additional results on the Gridworld environment in Appendix~\ref{additional_results}. 
The toy example above models several salient features in more complicated RL environments. 

(i) In the initial stages of learning, the exploratory policy is essentially random, and such a naive exploratory policy does not often lead to non-trivial rewards.

(ii)  Large positive and negative reward states (the goal and trap states), and their neighbors provide the pivot state for \namel~and \nameo.  

We show empirically that this holds in more complicated environments as well. Figure~\ref{fig:scatterplot_ant} depicts the surprise vs. reward for the Ant environment. Here we see a strong correlation between absolute reward and TD error (``Surprise factor'').

\begin{figure*}[hbt]
\centering
\subfigure[UER]{%
\includegraphics[width=0.3\linewidth]{figures/sparsity_new/ant_scatterplot_UER.pdf}
\label{fig:uer_ant_scatterplot}}
\subfigure[RER]{%
\includegraphics[width=0.3\linewidth]{figures/sparsity_new/ant_scatterplot_RER.pdf}
\label{fig:rer_ant_scatterplot}}
\subfigure[IER]{%
\includegraphics[width=0.3\linewidth]{figures/sparsity_new/ant_scatterplot_RER++.pdf}
\label{fig:rer++_ant_scatterplot}}


\caption{Relationship between absolute values of TD Error (Surprise factor) and Reward for the Ant environment.}
\label{fig:scatterplot_ant}
\end{figure*}

% \begin{figure}[hbt]
% \centering
% \subfigure[UER]{%
% \includegraphics[width=0.3\linewidth]{figures/scatterplot/ant_scatterplot_UER.pdf}
% \label{fig:uer_ant_scatterplot}}
% \subfigure[RER]{%
% \includegraphics[width=0.3\linewidth]{figures/scatterplot/ant_scatterplot_RER.pdf}
% \label{fig:rer_ant_scatterplot}}
% \subfigure[IER]{%
% \includegraphics[width=0.3\linewidth]{figures/scatterplot/ant_scatterplot_RER++.pdf}
% \label{fig:rer++_ant_scatterplot}}


% \caption{Relationship between TD Error (Surprise factor) and Reward for the Ant environment.}
% \label{fig:scatterplot_ant}
% \end{figure}


==> ICML_ IER/icml23/conclusion.tex <==
\section{Discussion}
\label{disc}
We summarize our results and discuss possible future steps.
%This section summarizes some of the exciting properties of \namel~discovered from our series of experiments in this paper. We also discuss some possible future steps. 
\paragraph{Speedup:} 
\namel~shows a significant speedup in terms of time complexity over \namep~as depicted in Table~\ref{tab:speedup}. On average \namel~achieves a speedup improvement of $26.20\%$ over \namep~across a large umbrella of environment classes.%Note that our algorithm's predominant time is spent computing the TD error of all samples in the buffer.
As the network becomes more extensive or complicated, our approach does have a higher overhead (especially computing TD error). Future work can investigate how to further reduce the computational complexity of our method by computing the TD error fewer times at the cost of operating with an older TD error. %This is highlighted from the results on Mujoco, where updating the sampling distribution using \namep~is faster than computing the TD error for all samples.
We also notice a speedup of convergence toward a local-optimal policy of our proposed approach, as shown in a few environments. Furthermore, the lack of speedup in some of the other experiments (even if they offer an overall performance improvement) could be since the "surprised" pivot cannot be successfully utilized to teach the agent rapidly in the initial stages. We refer to Appendix~\ref{additional_results} for the learning curves.  


\begin{table}[hbt!]
  \centering
  \caption{Average Speedup in terms of time complexity over \namep~across various environment classes.}
    \vspace*{1mm}
    
  \resizebox{0.4\columnwidth}{!}{
  \begin{tabular}{lc}
\toprule
\textbf{Environment} & {\textit{\textbf{Average Speedup}}}\\ \midrule
\midrule

\text{Classic Control}  & 32.66\% $\color{green}{\uparrow}$ \\ \midrule
\text{Box-2D} & 54.32\% $\color{green}{\uparrow}$ \\ \midrule
\text{Mujoco} & 18.09\% $\color{red}{\downarrow}$ \\  \midrule
\text{Robotics} & 55.56\% $\color{green}{\uparrow}$ \\ \midrule
\text{Atari} & 6.53\% $\color{green}{\uparrow}$ \\ 
\bottomrule
\end{tabular}
 }
\label{tab:speedup}
\end{table}

% \begin{wraptable}{C}{0.35\columnwidth}
% \centering
% \caption{Average Speedup in terms of time complexity over \namep~across various environment classes.}
% \vspace*{1mm}
% \label{tab:speedup}
% \resizebox{0.5\columnwidth}{!}{

% \begin{tabular}{lc}
% \toprule
% \textbf{Environment} & {\textit{\textbf{Average Speedup}}}\\ \midrule
% \midrule

% \text{Classic Control}  & 32.66\% $\color{green}{\uparrow}$ \\ \midrule
% \text{Box-2D} & 54.32\% $\color{green}{\uparrow}$ \\ \midrule
% \text{Mujoco} & 18.09\% $\color{red}{\downarrow}$ \\  \midrule
% \text{Robotics} & 55.56\% $\color{green}{\uparrow}$ \\ \midrule
% \text{Atari} & 6.53\% $\color{green}{\uparrow}$ \\ 
% \bottomrule
% \end{tabular}
% }
% \end{wraptable}

% \begin{table}[h!]
%   \centering
%   \resizebox{0.3\columnwidth}{!}{
%   \begin{tabular}{cc}
%     \toprule
%     \textbf{Environment} & {\textit{\textbf{Average Speedup}}}\\ \midrule
%     \midrule
  
%     \textit{Classic Control}  & 32.66\% $\color{green}{\uparrow}$ \\ \midrule
%     \textit{Box-2D} & 54.32\% $\color{green}{\uparrow}$ \\ \midrule
%     \textit{Mujoco} & 18.09\% $\color{red}{\downarrow}$ \\  \midrule
%     \textit{Robotics} & 55.56\% $\color{green}{\uparrow}$ \\ \midrule
%     \textit{Atari} & 6.53\% $\color{green}{\uparrow}$ \\ \midrule
%     \bottomrule
%   \end{tabular}
%  }
%  \caption{Average Speedup in terms of time complexity over \namep~across various environment classes.}
%   \label{tab:speedup}
% \end{table}



% \rk{need to rewrite the paragraph below, given that we have sent the learning curves to the appendix. Add points about speeding up convergence to the optimal policy. However, only if there is hard evidence of this.}
% Furthermore, even if we notice a similar speedup in some cases of \namep, the number of CPU hours (in the case of CartPole) used is almost ten times more. 
% To conclude, the core of \namel~is in line with our intuition that looking back when surprised does teach the model a lot during the initial few steps of the learning. 
\paragraph{Issues with stability and consistency} 

Picking pivot points by looking at the TD error might cause us to sample rare events much more often and hence cause instability compared to \nameu~as seen in some environments like HalfCheetah, LunarLander, and Ant, where there is a sudden drop in performance for some episodes (see Appendix~\ref{additional_results}). We observe that our strategy \namel~corrects itself quickly, unlike \namelo, which cannot do this (see Figure~\ref{fig:lr_hopper}). Increasing the number of pivot points per episode (the parameter $G$) and the uniform mixing probability $p$ usually mitigates this. In this work, we do not focus on studying the exact effects of $p$ and $G$ since our objective was to obtain methods that require minimal hyper-parameter tuning. However, future work can systematically investigate the significance of these parameters in various environments.

% \rk{Shall we break this into two parts, one for discussion and another for the conclusion? It would be nice to remind the short-term memory reviewers what we did in the paper.}

% It would be interesting to explore gradually mixing \namel~with some form of uniformly random pivot-picking strategy in order to obtain the best of both worlds. From additional experiments (see Figure ~\ref{fig:urer++}), we show that the self-correcting instability concerns, although rare, could be mitigated by infusing random sampling of pivots or batches with \namel. Here, although the \namel~agent seems to learn beneficial properties towards the end of the training, the phenomenon is highly seed-dependent and not dependable for robust learning. In this experiment, we use a sampler called \nameul, where we use \namel~with a probability of 70\% and \nameu~with a probability of 30\% while sampling each buffer. This intuition has been previously explored by \cite{rotinov2019reverse}, although their proposed approach involved combining \nameu~with \namelo~instead of \namel. Even with a simple ad-hoc solution, as mentioned earlier, we could successfully mitigate the instability concerns of \namel. Figure~\ref{fig:urer++} depicts the learning curve in the increased gradient steps setting for the Hopper environment. Table~\ref{tab:inc_steps} summarizes our findings as a moving average metric with a window size of 50.
% \rk{connect to hopper experiment}

\paragraph{Why does \namel~outperform the traditional \namelo?}
The instability\footnote{i.e., sudden drop in performance without recovery like catastrophic forgetting} and unreliability of pure \namelo~with neural approximation has been noted in various works \citep{rotinov2019reverse,lee2019sample}, where \namelo~is stabilized by mixing it with \nameu~. \cite{hong2022topological} stabilizes reverse sweep by mixing it with \namep. This is an interesting phenomenon since RER is near-optimal in the tabular and linear approximation settings \citep{agarwal2021online}. Two explanations of this are i) The loss function used to train the neural network is highly non-convex, which hinders the working of \namelo~and ii) The proof given in \cite{agarwal2021online} relies extensively on `coverage' of the entire state-action space - that is, the entire state-action space is visited enough number of times - which might not hold, as shown in the toy example in Section~\ref{sec:toy_example}.


%Naively going in the reverse order inside a buffer might be sub-optimal due to the highly non-convex nature of the neural network loss landscape. It is also computationally intractable to pass through the entire buffer for neural networks. 


\section{Conclusion}

In conclusion, our proposed approach, Introspective Experience Replay (\namel), has shown significant promise as a solution for improving the convergence and robustness of reinforcement learning algorithms. We have demonstrated through extensive experiments that \namel~outperforms state-of-the-art techniques such as uniform experience replay (\nameu), prioritized experience replay (\namep), and hindsight experience replay (\nameh) on a wide range of tasks, and also shows a significant average speedup improvement in terms of time complexity over \namep. One of the key strengths of our proposed approach is its ability to selectively sample batches of data points prior to surprising events. This allows for the removal of bias and spurious correlations that can impede the convergence of RL algorithms. Additionally, our method is based on the theoretically rigorous reverse experience replay (\namelo) technique, which adds a further level of rigor to our approach.

Overall, our proposed approach, Introspective Experience Replay (\namel), is a promising solution that offers significant improvements over existing methods and has the potential to advance the field of reinforcement learning. We believe that our proposed approach could be widely adopted in various RL applications and have a positive impact on the field of AI.

==> ICML_ IER/icml23/introduction.tex <==
\section{Introduction}
% \dn{Other Title ideas: Reverse Experience Replay for Neural Approximation/Neural Networks}
% \dn{What's in the traversal order for Experience Replay? }
% \dn{Hindsight is 20/20: A stable version of Reverse Experience Replay }
% \rk{For the intro, we have these two things to work on:
% 1. We claim PER incurs large bias - we need to cite their paper that OER itself has bias and then claim from our experiments that even this fix doesn't work all the time outside Atari games in the original paper. 
% 2. Define what instability is and what sub-optimality is. See if RER can be called "unstable."
% We need to fix this language (instability vs sub-optimality) in the whole paper}

% \rk{ the paper mentions that previous methods have bias as one of their main weaknesses but does not show that their method is unbiased. }

% \rk{Similarly problematic is the use of the terms optimal or sub-optimal, which are defined and used in non-standard ways.}

Reinforcement learning (RL) involves learning with dependent data derived from trajectories of Markov processes. In this setting, the iterations of descent algorithms designed for i.i.d. data co-evolve with the trajectory at hand, leading to poor convergence. Experience replay \citep{lin1992self} involves storing the received data points in a large buffer and producing a random sample from this buffer whenever the learning algorithm requires it. Therefore experience replay is usually deployed with popular algorithms like DQN, DDPG, and TD3 to achieve state-of-the-art performance \citep{mnih2015human,lillicrap2015continuous}. It has been shown experimentally \citep{mnih2015human} and theoretically \citep{bresler2020least} that these learning algorithms for Markovian data show sub-par performance without experience replay. 

The simplest and most widely used experience replay method is the uniform experience replay (\nameu), where the data points stored in the buffer are sampled uniformly at random every time a data point is queried \citep{mnih2015human}. However, \nameu~might pick uninformative data points most of the time, which may slow down the convergence. For this reason, optimistic experience replay (\nameo) and prioritized experience replay (\namep)~\citep{schaul2015prioritized} were introduced, where samples with higher TD error (i.e., `surprise') are sampled more often from the buffer. Optimistic experience replay (originally called ``greedy TD-error prioritization'') was shown to have a high bias\footnote{We use the term `bias' here as used in \cite{schaul2015prioritized}, which means biased with respect to the empirical distribution over the replay buffer}. This leads to the algorithm predominantly selecting rare data points and ignoring the rest. Prioritized experience replay was proposed to solve this issue \citep{schaul2015prioritized} by using a sophisticated sampling approach. However, as shown in our experiments outside of the Atari environments, \namep~still suffers from a similar problem, and its performance can be highly sensitive to seed and hyper-parameter. Although this speeds up the learning process in many cases, its performance can be quite bad and erratic due to picking and choosing only specific data points. The design of experience replay continues to be an active field of research. Several other experience replay techniques like Hindsight experience replay (\nameh)~\citep{andrychowicz2017hindsight}, Reverse Experience Replay (\namelo)~\citep{rotinov2019reverse}, and Topological Experience Replay (\namet)~\citep{hong2022topological} have been proposed. An overview of these methods is discussed in Section~\ref{rel_works}. 

%Several specialized methods have been proposed and evaluated experimentally from the simplest form of experience replay as used in \cite{mnih2015human}, where uniform sampling from a buffer is used (\nameu). 
%These include prioritized experience replay (\namep)~\citep{schaul2015prioritized}, 
%hindsight experience replay (\nameh)~\citep{andrychowicz2017hindsight}, reverse experience replay (\namelo)~\citep{rotinov2019reverse}, and% topological experience replay (\namet)~\citep{hong2022topological}. 

Even though these methods are widely deployed in practice, theoretical analyses have been very limited. Recent results on learning dynamical systems \citep{kowshik2021streaming,kowshik2021near} showed rigorously in a theoretical setting that \namelo~is the conceptually-grounded algorithm when learning from Markovian data. Furthermore, this work was extended to the RL setting in \cite{agarwal2021online} to achieve efficient Q learning with linear function approximation. The \namelo~technique achieves good performance since reverse order sampling of the data points prevents the build-up of spurious correlations in the learning algorithm. In this paper, we build on this line of work and introduce \textbf{Introspective Experience Replay} (\namel). Roughly speaking, \namel~first picks top $k$ `pivot' points from a large buffer according to their TD error. It then returns batches of data formed by selecting the consecutive points \emph{temporally} before these pivot points. In essence, the algorithm \emph{looks back when surprised}. The intuition behind our approach is linked to the fact that the agent should always associate outcomes to its past actions, just like in \namelo. The summary of our approach is shown in Figure~\ref{fig:rer++}. This technique is an amalgamation of Reverse Experience Replay (\namelo) and Optimistic Experience Replay (\nameo), which only picks the points with the highest TD error. 
% In the rest of this work, we first define the \namel~method and investigate its properties conceptually and experimentally against various benchmarks. Our study demonstrates that \namel~outperforms state-of-the-art methods in multiple environments justifies our design methodology via ablation studies, and gives evidence for our conceptual understanding via a simple toy example.

 
 
 %However, \namelo~seems unstable (not converging to a good policy) when used with neural function approximation (see Table~\ref{table:ablation}). 

%Our work modifies \namelo, namely \namel, which is stable when used with neural function approximation and outperforms other state-of-the-art replay methods over a diverse range of environments. Roughly speaking, \namelo~first picks top $k$ `pivot' points from a large buffer according to their TD error. It then returns batches of data formed by selecting the consecutive points \emph{temporally} before these pivot points. In essence, the algorithm \emph{looks back when surprised}. The intuition behind our approach is linked to the fact that the agent should always associate positive and negative lessons from its past actions. The summary of our approach is shown in Figure~\ref{fig:rer++}. 

\begin{figure}[hbt!]
\centering
\includegraphics[width=0.99\linewidth]{figures/rer++.pdf}
\label{fig:rer++}
\caption{An illustration of our proposed methodology when selecting $k$ batches in the CartPole environment. The red color is used to indicate the batches being sampled from the replay buffer. The green samples are the un-sampled states from the buffer. The arrow explicitly points the pivots and the snapshot of the surprising state encountered.}
\label{fig:ro}
\end{figure}




% It is well known that naive importance sampling (i.e., picking examples with the most significant TD error to form a minibatch) or using temporally consecutive data points (i.e., creating mini-batches with data points that are temporally adjacent) are both extremely ineffective \citep{schaul2015prioritized, mnih2013playing}. The former procedure, which we shall call optimistic experience replay (\nameo), incurs a significant bias error as discussed in \cite{schaul2015prioritized}, which is why \namep~uses a sophisticated sampling procedure to mitigate such a bias. Surprisingly, our algorithm combines these ineffective heuristics and works very well. One possible explanation of this phenomenon is that due to the de-biasing nature of \namelo~(see \cite{kowshik2021streaming}), even this naive importance selection in \namel~is efficient. 
Our main findings are summarized below:

\textbf{Better Performance Against SOTA:}
Our proposed methodology (\namel) outperforms previous state-of-the-art baselines such as \namep, \nameu~and \nameh~on most environments (see Table~\ref{tab:initial_results}, Section~\ref{results}).

\textbf{Conceptual Understanding:} We consider a simple toy example where we understand the differences between \nameu, \namelo, \nameo~and \namel~(Section~\ref{sec:toy_example}). This study illustrates the better performance of our proposed method by showing a) why naive importance sampling, like in \nameo~suffers from poor performance, often failing to learn any non-trivial policy and b) why techniques like \nameu~and \namelo~are slow to learn. 

\textbf{Forward vs. Reverse:} We show that the temporal direction (forward/reverse) to consider after picking the pivot is non-trivial. We show empirically that \namel~performs much better than its forward counterpart, IER (F) (see Table~\ref{table-temporl-results}). This gives evidence that causality plays a role in the success of \namel. 

\textbf{Whole vs. Component Parts:} Our method (\namel) is obtained by combining two methods \namelo~(which picks the samples in the reverse order as received) and \nameo~(which greedily picks the samples with the largest TD error). We show that neither of these components performs well compared to their amalgamation, \namel~(Table~\ref{table:ablation}). 
%\dn{ not sure we should point this out: Although reinforcement learning is highly seed-dependent, especially when working with experience replay, our proposed methodology has a much lower error bound than other baselines. (Section~\ref{results})}
%\paragraph{Time Complexity:} Our proposed methodology has a significantly lower time complexity than \namep and shows speedup on various environments, including Classic control, Box 2D, Robotics, and Atari. (Table~\ref{tab:speedup})

\textbf{Minimal hyperparameter tuning:} Our proposed methodology uses minimal hyperparameter tuning. We use the same policy network architecture, learning rate, batch size, and all other parameters across all our runs for a given environment. These hyperparameters are selected based on the setting required to achieve SOTA performance on \nameu. However, we have few options available, a \textit{Hindsight} flag, leading to the H-IER sampler, and the \textit{Uniform Mixing fraction} leading to the \nameul~sampler. Furthermore, for most of our experiments, we use a mixing fraction of $0$.

\begin{table}[!hbt]\centering
    \vspace{-10pt}
\caption{\textbf{\namel~outperforms previous state-of-the-art baselines}. These baselines include samplers such as \nameu~\citep{mnih2013playing}, \namep~\citep{schaul2015prioritized}, and \nameh~\citep{andrychowicz2017hindsight} across many environments. Results are from 13 different environments that cover a broad category of MDPs. These include a few Atari environments (previously used to support the efficacy of \nameu, \namep), some Robotics environments (previously used to support the efficacy of \nameh), and many other classes of environments, including Classic Control, Box 2D, and Mujoco. More details about these experiments and their setup have been discussed in Section~\ref{results}.
}
\vspace*{1mm}
\label{tab:initial_results}
\resizebox{0.8\linewidth}{!}{
\begin{tabular}{lcccc}
\toprule
% \hline
Experience Replay Method & {UER} & {PER} & {HER} & {IER} \\ \midrule
Best Performance Frequency & 1 & 0 & 1  & {\color[HTML]{3166FF} \textbf{11}}\\ \bottomrule
\end{tabular}
}
    \vspace{-10pt}
\end{table}


==> ICML_ IER/icml23/related_works.tex <==
\section{Related Works and Comparison}
\label{rel_works}
\subsection{Experience Replay Techniques}
Experience replay involves storing consecutive temporally dependent data in a (large) buffer in a FIFO order. Whenever a learning algorithm queries for batched data, the experience replay algorithm returns a sub-sample from this buffer such that this data does not hinder the learning algorithms due to spurious correlations. The most basic form of experience replay is \nameu~\citep{lin1992self} which samples the data in the replay buffer uniformly at random. This approach has significantly improved the performance of off-policy RL algorithms like DQN \citep{mnih2015human}. Several other methods of sampling from the buffer have been proposed since; \namep~\citep{schaul2015prioritized} samples experiences from a probability distribution which assigns higher probability to experiences with significant TD error and is shown to boost the convergence speed of the algorithm. This outperforms \nameu~in most Atari environments. \nameh~\citep{andrychowicz2017hindsight} works in the "what if" scenario, where even a bad policy can lead the agent to learn what not to do and nudge the agent towards the correct action. There have also been other approaches such as \cite{liu2019competitive, fang2018dher, fang2019curriculum} have adapted \nameh~in order to improve the overall performance with varying intuition.
\namelo~processes the data obtained in a buffer in the reverse temporal order. We refer to the following sub-section for a detailed review of this and related techniques. We will also consider `optimistic experience replay' (OER), the naive version of \namep, where at each step, only top $B$ elements in the buffer are returned when batched data is queried. This approach can become highly selective to the point of completely ignoring certain data points, leading to poor performance. This is mitigated by a sophisticated sampling procedure employed in \namep. Other works such as \cite{fujimoto2020equivalence, pan2022understanding} attempt to study \namep~and address some of its shortcomings, and \cite{lahire2021large} introduces 'large batch experience replay' (LaBER), which reduces the stochastic noise in gradients while keeping the updates unbiased with respect to the empirical data distribution in the replay buffer 

\subsection{Reverse Sweep Techniques}
\label{sec:rev_sweep}
Reverse sweep or backward value iteration refers to methods that process the data as received in reverse order. This has been studied in the context of planning tabular MDPs \citep{dai2007prioritizing,grzes2013convergence}. We refer to Section~\ref{understanding_rer} for a brief overview of why these methods are considered. However, this line of work assumes that the MDP and the transition functions are known. Inspired by the behavior of biological networks, \cite{rotinov2019reverse} proposed reverse experience replay where the experience replay buffer is replayed in a LIFO order. Since \namelo~forms mini-batches with consecutive data points can be unreliable with Neural approximation (i.e., it does not learn consistently well across different environments). Therefore, the iterations of \ namelo~are `mixed' with \nameu. However, the experiments are limited and do not demonstrate that this method outperforms even \nameu. A similar procedure named Episodic Backward Update (EBU) is introduced in \cite{lee2019sample}. However, to ensure that the pure \namelo~works well, the EBU method also seeks to change the target for Q learning instead of just changing the sampling scheme in the replay buffer.
The reverse sweep was independently rediscovered as \namelo~in the context of streaming linear system identification in \cite{kowshik2021streaming}, where SGD with reverse experience replay was shown to achieve near-optimal performance. In contrast, naive SGD was significantly sub-optimal due to the coupling between the Markovian data and the SGD iterates. The follow-up work \cite{agarwal2021online} analyzed off-policy Q learning with linear function approximation and reverse experience replay to provide near-optimal convergence guarantees using the unique super martingale structure endowed by reverse experience replay. 
\cite{hong2022topological} considers topological experience replay, which executes reverse replay over a directed graph of observed transitions. Mixed with \namep~enables non-trivial learning in some challenging environments. Another line of work \citep{florensa2017reverse,moore1993prioritized,goyal2018recall,schroecker2019generative} considers reverse sweep with access to a simulator or using a fitted generative model. On the other hand, our work only seeks on-policy access to the MDP.



==> ICML_ IER/icml23/results.tex <==
\section{Experimental Results}
\label{results}

In this section, we briefly discuss our experimental setup as well as the results of our experiments.
\paragraph{Environments:} We evaluate our approach on a diverse class of environments, such as (i) Environments with low-dimensional state space (including classic control and Box-2D environments), (ii) Multiple joint dynamic simulations and robotics environments (including Mujoco and Robotics environments), and (iii) Human-challenging environments (such as Atari environments). Note that previous seminal papers in the field of experience replay, such as \cite{mnih2013playing}, \cite{schaul2015prioritized}, and \cite{andrychowicz2017hindsight}, showed the efficacy of their approach on a subset of these classes. For instance, \nameu and \namep~was shown to work well on Atari games. Furthermore, \nameh~was effective in the Robotics environments such as FetchReach. In this work, we perform a more extensive study to show the robustness and effectiveness of our model not just in Atari and Robotics environments but also in Mujoco, Box2D, and Classic Control environments. Due to computational limitations and the non-reproducibility of some baselines, we could not extend our experiments to some Atari environments. We refer to Appendix~\ref{appendix-env} for a brief description of the environments used.

\paragraph{Hyperparameters:}
Refer to Appendix~\ref{appendix-hyperparam} for the exact hyperparameters used. Across all our experiments on various environments, we use a standard setting for all the different experience replay buffers. This classic setting is set so we can reproduce state-of-the-art performance using \nameu~on the respective environment. For most of our experiments, we set the uniform mixing fraction ($p$) from Algorithm~\ref{alg:rev_plus} to be 0. We use a non-zero $p$ value only for a few environments to avoid becoming overtly selective while training, as described in Appendix~\ref{appendix-hyperparam}. For \namep, we tune the $\alpha$ and $\beta$ hyperparameters used in the \cite{schaul2015prioritized} paper across all environments other than Atari. The default values of $\alpha=0.4$ and $\beta=0.6$ are robust on Atari environments as shown by extensive hyperparameter search by \cite{schaul2015prioritized}. We detail the results from our grid search in Appendix~\ref{appendix:per_grid_search}.

% , \rk{0.5 for Pendulum, 0.4 for Walker,} and 0.3 for HalfCheetah. 

\paragraph{Metric:} To compare the different models, we use the \textit{Top-K seeds moving average return} as the evaluation metric across all our runs. Top-K seeds here mean we take the average of $k=3$ seeds that gave the best performance out of a total of $n=5$ trials. This measures the average performance of the top $k/n$ quantile of the trajectories. This factors in the seed sensitivity and is robust despite the highly stochastic learning curves encountered in RL, where there is a non-zero probability that non-trivial policies are not learned after many steps. It is common to use top-1 and Top-K trials to be selected from among many trials in the reinforcement learning literature (see \cite{schaul2015prioritized};\cite{sarmad2019rl};\cite{wu2017scalable};\cite{mnih2016asynchronous}). Furthermore, we motivate our design choice of using the Top-K metric as our metric of choice from our study in Appendix~\ref{appendix:metrics}. We show that the Top-K metric is more stable and suitable for comparing the performances of different RL agents, which generally suffer from highly volatile learning curves, as described above. 
Moving average with a given window size is taken for learning curves (with a window size of 20 for FetchReach and 50 for all others) to reduce the variation in return which is inherently present in each epoch. We argue that taking a moving average is essential since, usually, pure noise can be leveraged to pick a time instant where a given method performs best \citep{henderson2018deep}. Considering the Top-K seed averaging of the last step performance of the moving average of the learning curves gives our metric - the \textit{Top-K seeds moving average return}.
%Across all the environments other than FetchReach, we use a running average of 50 timesteps for robust estimation and visualization. However, we use a window size of 20 for the FetchReach environment since these experiments were run for a significantly lower number of epochs.

\paragraph{Comparison with SOTA:} Table~\ref{table-results_1} depicts our results in various environments upon using different SOTA replay sampler mechanisms (\nameu, \namep~and \nameh). Our proposed sampler outperforms all other baselines in most tasks and compares favorably in others. Our experiments on various environments across various classes, such as classic control, and Atari, amongst many others, show that our proposed methodology consistently outperforms all other baselines in most environments, as summarized in Table~\ref{tab:initial_results}. Furthermore, our proposed methodology is robust across various environments, as highlighted in Table~\ref{table-results_1}. The learning curves for our experiments have been depicted in the Appendix. (see Appendix~\ref{additional_results})

\begin{table}[hbt!]
  \centering
  \caption{\textit{Top-K seeds Moving Average Return} results across various environments. From our experiments, we note that \namel~outperforms previous SOTA baselines in most environments. Appendix~\ref{appendix-hyperparam} depicts the hyperparameters used for the experiment.}
  \vspace*{1mm}
  \label{table-results_1}
  \resizebox{\columnwidth}{!}{
  \begin{tabular}{lcccc}  
    \toprule
    \textbf{Dataset} & {\textit{\textbf{UER}}} & {\textit{\textbf{PER}}}  & {\textit{\textbf{HER}}}  & {\textit{\textbf{IER}}} \\ \toprule
    {\text{CartPole}}  & 153.14 {\tiny $\pm$ 32.82} & 198.06 {\tiny $\pm$ 3.68} & 173.84 {\tiny $\pm$ 26.11} & \textbf{199.83} {\tiny $\pm$ 0.31}\\  \midrule
    
    {\text{Acrobot}} & -257.93 {\tiny $\pm$ 184.28} & -233.45 {\tiny $\pm$ 127.99} & -389.42 {\tiny $\pm$ 113.22} & \textbf{-193.90} {\tiny $\pm$ 57.56} \\  \midrule
    
    {\text{Inverted Pendulum}} & -161.93 {\tiny $\pm$ 10.55} & -155.05 {\tiny $\pm$ 9.95} & -629.42 {\tiny $\pm$ 815.24} & \textbf{-150.27} {\tiny $\pm$ 9.63} \\  \midrule
    
    {\text{LunarLander}}  & -4.42 {\tiny $\pm$ 20.06} & 11.21 {\tiny $\pm$ 15.51} & 6.00 {\tiny $\pm$ 10.02} & \textbf{12.32} {\tiny $\pm$ 27.55}\\  \midrule
    
    {\text{HalfCheetah}}  & 10808.93 {\tiny $\pm$ 1094.32} & 99.75 {\tiny $\pm$ 1124.46} & \textbf{11072.54} {\tiny $\pm$ 297.12} & 10544.88 {\tiny $\pm$ 342.01}\\  \midrule
    
    {\text{Ant}}  & 3932.85 {\tiny $\pm$ 1024.86} & -2699.84 {\tiny $\pm$ 1.34} & 3803.17 {\tiny $\pm$ 996.81}  & \textbf{4203.21} {\tiny $\pm$ 345.22}\\  \midrule
    
    {\text{Reacher}}  & -4.97 {\tiny $\pm$ 0.31} & -5.42 {\tiny $\pm$ 0.61} & -5.30 {\tiny $\pm$ 0.50}  & \textbf{-4.92} {\tiny $\pm$ 0.27}\\  \midrule
    
    {\text{Walker}}  & 3597.03 {\tiny $\pm$ 1203.79} & 1709.48 {\tiny $\pm$ 1635.90} & 889.82 {\tiny $\pm$ 1427.92}  & \textbf{4349.29} {\tiny $\pm$ 680.35}\\  \midrule
    
    {\text{Hopper}}  & 3072.65 {\tiny $\pm$ 621.40} & 784.00 {\tiny $\pm$ 1536.00} & 2685.72 {\tiny $\pm$ 1221.81} & \textbf{3205.05} {\tiny $\pm$ 406.35} \\  \midrule
    
    {\text{Inverted Double Pendulum}} & 8489.54 {\tiny $\pm$ 927.69} & 8654.78  {\tiny $\pm$ 981.67} & 9002.05 {\tiny $\pm$ 464.20} & \textbf{9241.61} {\tiny $\pm$ 91.68}\\  \midrule
    % \textbf{9067.69} {\tiny $\pm$ 402.39}\\  \midrule
    
    {\text{Fetch-Reach}}  & -1.84 {\tiny $\pm$ 0.57} & -49.90 {\tiny $\pm$ 0.10} & -2.92 {\tiny $\pm$ 1.79} &  \textbf{-1.74} {\tiny $\pm$ 0.24}\\  \midrule
    
    {\text{Pong}} & \textbf{19.15} {\tiny $\pm$ 1.32} & 17.02 {\tiny $\pm$ 3.27} & 18.70 {\tiny $\pm$ 1.02} & 19.10 {\tiny $\pm$ 1.20}\\  \midrule
    
    {\text{Enduro}} & 227.01 {\tiny $\pm$ 319.15} & 565.23 {\tiny $\pm$ 116.36} & 514.32 {\tiny $\pm$ 132.39} & \textbf{586.32} {\tiny $\pm$ 111.44} \\
    \bottomrule
  \end{tabular}
 }
\end{table}



\paragraph{Forward vs. Reverse:} The intuitive limitation to the "looking forward" approach is that in many RL problems, the objective for the agent is to reach a final goal state, where the non-trivial reward is obtained. Since non-trivial rewards are only offered in this goal state, it is informative to look back from here to learn about the states that \emph{lead} to this. When the goals are sparse, the TD error is more likely to be large upon reaching the goal state. Our algorithm selects these as pivots, and IER (F) might select batches overflowing into the next episode. Our studies on many environments (see Figure~\ref{fig:scatterplot_ant} and Appendix~\ref{sparse_surprise}) show that the pivot points selected based on importance indeed have large (positive or negative) rewards. Our experiments depicted in Table~\ref{table-temporl-results} show that \namel~outperforms IER (F) in most environments.

\begin{table}[h!]
  \centering
  \caption{\textit{Top-K seeds Moving Average Return} results across various environments for Temporal Ablation study between IER (F) and IER (R; default). Note that we use the base setting of \namel~in this section to avoid spurious comparisons (i.e., with $p = 0$ and no hindsight).}
  \vspace*{1mm}
  \label{table-temporl-results}
  \resizebox{0.7\columnwidth}{!}{
  \begin{tabular}{lcc}
    \toprule
    \textbf{Dataset} & {\textit{\textbf{Forward}}} & {\textit{\textbf{Reverse}}} \\ \toprule
    {\text{CartPole}}  & 196.51 {\tiny $\pm$ 6.26} & \textbf{199.83} {\tiny $\pm$ 0.31}\\  \midrule
    
    {\text{Acrobot}} & -423.15 {\tiny $\pm$ 108.08} & \textbf{-313.03} {\tiny $\pm$ 190.27}\\  \midrule
    
    {\text{Inverted Pendulum}} & \textbf{-882.13} {\tiny $\pm$ 521.77} & -1111.51 {\tiny $\pm$ 559.83}\\  \midrule
    
    {\text{LunarLander}}  & -22.75 {\tiny $\pm$ 30.19} & \textbf{12.32} {\tiny $\pm$ 27.55}\\  \midrule
    
    {\text{HalfCheetah}}  & 9369.30 {\tiny $\pm$ 454.40} & \textbf{10108.15} {\tiny $\pm$ 919.27}\\  \midrule
    
    {\text{Ant}}  & 2963.71 {\tiny $\pm$ 828.50} & \textbf{4203.21} {\tiny $\pm$ 345.22}\\  \midrule
    
    {\text{Reacher}}  & -5.25 {\tiny $\pm$ 0.33} & \textbf{-4.92} {\tiny $\pm$ 0.27}\\  \midrule
    
    {\text{Walker}}  & 2213.89 {\tiny $\pm$ 1684.03} & \textbf{2830.03} {\tiny $\pm$ 881.51}\\  \midrule
    
    {\text{Hopper}}  & 393.64 {\tiny $\pm$ 181.89} & \textbf{505.58} {\tiny $\pm$ 266.52}\\  \midrule
    
    {\text{Inverted Double Pendulum}} & \textbf{9260.27} {\tiny $\pm$ 95.59} & \textbf{9241.61} {\tiny $\pm$ 91.68} \\ \midrule
    % 9067.69 {\tiny $\pm$ 402.39}\\  \midrule
    
    {\text{FetchReach}}  & -17.73 {\tiny $\pm$ 27.91} & \textbf{-2.28} {\tiny $\pm$ 1.11}\\  \midrule
    
    {\text{Pong}}  & 17.92 {\tiny $\pm$ 2.60} & \textbf{19.10} {\tiny $\pm$ 1.20}\\  \midrule

    {\text{Enduro}}  & \textbf{600.87} {\tiny $\pm$ 149.99} & 525.84 {\tiny $\pm$ 146.39} \\
    \bottomrule
  \end{tabular}
 }
\end{table}



\paragraph{Whole vs. Component Parts:} Our approach is an amalgamation of \nameo~and \namelo. Here we compare these individual parts with \namel. Table~\ref{table:ablation} describes the \textit{Top-K seeds Moving Average Return} across various environments in this domain. As demonstrated, \namel~outperforms its component parts \nameo~nor \namelo~. Furthermore, we also motivate each of our design choices such as the pivot point selection (see Appendix~\ref{pivot_ablation} where we compare our proposed approach with it's variant where the pivot points are randomly selected), and temporal structure (see Appendix~\ref{lookingback_ablation} where we compare our proposed approach with it's variant where the points are randomly sampled instead of temporally looking backward after selecting a pivot point, and also buffer batch size sensitivity (see Appendix~\ref{buffer_size_ablation}).

\begin{table}[hbt!]
  \centering
  \caption{\textit{Top-K seeds Moving Average Return} results across various environments for ablation study between \namelo, \nameo, and \namel.}
  \vspace*{1mm}
  \resizebox{0.8\columnwidth}{!}{
  \begin{tabular}{lccc}  
    \toprule
    \textbf{Dataset} &  {\textit{\textbf{RER}}}  & {\textit{\textbf{OER}}}  & {\textit{\textbf{IER}}} \\ \toprule
    {\text{CartPole}}  & 163.93 {\tiny $\pm$ 40.03} & 162.36 {\tiny $\pm$ 34.89} & \textbf{199.83} {\tiny $\pm$ 0.31}\\  \midrule
    
    {\text{Acrobot}} & -320.70 {\tiny $\pm$ 144.05} & -472.63 {\tiny $\pm$ 31.21} & \textbf{-193.90} {\tiny $\pm$ 57.56} \\  \midrule
    
    {\text{Inverted Pendulum}} & -735.38 {\tiny $\pm$ 613.5} & -166.57 {\tiny $\pm$ 17.23} & \textbf{-150.27} {\tiny $\pm$ 9.63} \\  \midrule
    
    {\text{LunarLander}}  & 9.84 {\tiny $\pm$ 13.23} & -16.08 {\tiny $\pm$ 15.38} & \textbf{12.32} {\tiny $\pm$ 27.55}
    \\\midrule
    
    {\text{HalfCheetah}}  & 9449.39 {\tiny $\pm$ 648.60} & 2237.91 {\tiny $\pm$ 2824.72} & \textbf{10544.88} {\tiny $\pm$ 342.01}\\  \midrule
    
    {\text{Ant}}  & 2168.47 {\tiny $\pm$ 415.53} & -47.93 {\tiny $\pm$ 20.47} & \textbf{4203.21} {\tiny $\pm$ 345.22}\\  \midrule
    
    {\text{Reacher}}  & -5.91 {\tiny $\pm$ 0.37} &  -5.28 {\tiny $\pm$ 0.58} & \textbf{-4.92} {\tiny $\pm$ 0.27} \\  \midrule
    
    {\text{Walker}}  & 1578.33 {\tiny $\pm$ 1313.11} & 207.51 {\tiny $\pm$ 193.06} & \textbf{4349.29} {\tiny $\pm$ 680.35} \\  \midrule
    
    {\text{Hopper}}  & 206.23 {\tiny $\pm$ 318.49} & 660.24 {\tiny $\pm$ 580.77} & \textbf{3205.05} {\tiny $\pm$ 406.35} \\  \midrule
    
    {\text{Inverted Double Pendulum}} & 8953.44 {\tiny $\pm$ 456.95} & 7724.99 {\tiny $\pm$ 1726.58} & \textbf{9241.61} {\tiny $\pm$ 91.68}\\ \midrule
    % \textbf{9067.69} {\tiny $\pm$ 402.39}\\  \midrule
    
    {\text{Fetch-Reach}}  & -49.94 {\tiny $\pm$ 0.07} & -47.72 {\tiny $\pm$ 3.33} & \textbf{-1.74} {\tiny $\pm$ 0.24}\\  \midrule
    
    {\text{Pong}} & 18.58 {\tiny $\pm$ 1.75} & 3.52 {\tiny $\pm$ 21.33} & \textbf{19.10} {\tiny $\pm$ 1.20}\\  \midrule
    
    {\text{Enduro}} & 483.98 {\tiny $\pm$ 75.45} & 361.21 {\tiny $\pm$ 86.30} & \textbf{586.32} {\tiny $\pm$ 111.44} \\
    \bottomrule
  \end{tabular}
 }
\label{table:ablation}
\end{table}


% \rk{Do we want to add a section studying "the number of steps taken to reach a given average return"? This might become useful to show improvements over RER. RER will implicitly need more steps just because it needs to cover the entire buffer, whereas RER++ can sample the important points and achieve faster/hopefully better performance across the board.}

% \rk{HRER++ has not been discussed in Section~\ref{disc} as claimed. Perhaps add a short note in the algorithms section itself}
% From Figure~\ref{fig:ablation_study}, we note that \namelo~and \nameo~are not very competitive and do not farewell. However, the amalgamation of the intuitions from the two concepts fits very well and results in a highly competitive methodology across many environments.


==> ICML_ IER/icml23/toy_example.tex <==
\section{Understanding Reverse Replay}
\label{understanding_rer}
There are various conceptual ways we can look at \namelo~and \namel. This section outlines some of the motivations behind using this technique. Theoretical works such as \cite{agarwal2021online,kowshik2021streaming} have established rigorous theoretical guarantees for \namelo~by utilizing super martingale structures. This structure is not present in forward replay techniques (i.e., the opposite of reverse replay) as shown in \cite{kowshik2021near}. We refer to Appendix~\ref{ablation_temporal}, where we show via an ablation study that going forward in time instead of reverse does not work very well. We give the following explanations for the success of \namel. \newline
 %   \paragraph{Super Martingale Structure in Descent Algorithms:}
    % As was noted in \cite{kowshik2021streaming} in the linear system identification setting, processing Markov process data in the order they are received through SGD-like algorithms can lead to biases that cause sub-optimal performance. However, simply processing the received data in reverse order with \namelo~can remove these biases by leveraging specific super-martingale structures. These observations were later extended to the non-linear and RL settings in \cite{kowshik2021near,agarwal2021online}.
    % \paragraph{Dynamic Programming:} Dynamic programming algorithms are some of the first computationally efficient algorithms established for RL \cite{bertsekas1995neuro}. Here again, the optimal policy is constructed by going backward in time to avoid exponential dependence on the horizon incurred by the brute force algorithm. Indeed, this is the idea behind reverse sweep or backward value iteration in \cite{dai2007prioritizing,grzes2013convergence}, which mainly deals with planning when the MDP itself is fully known.
\textbf{Propogation of Sparse Rewards:} In many RL problems, non-trivial rewards are sparse and only received at the goal states. Therefore, processing the data backward in time from such goal states helps the algorithm learn about the states that led to this non-trivial reward. Our study (see Figure \ref{fig:scatterplot_ant} and Appendix~\ref{sparse_surprise} for further details) shows that in many environments \namel~picks pivots which are the states with large (positive or negative) rewards, enabling effective learning. \newline
\textbf{More spread than \nameo:} \nameo, which greedily chooses the examples with the largest TD error to learn from, performs very poorly since it is overtly selective to the point of ignoring most of the states. To illustrate this phenomenon, we refer to the didactic example in Section~\ref{sec:toy_example}. One possible way of viewing \namel~is that \namelo~is used to reduce this affinity to picking a minimal subset of states in \nameo. \namep~is designed to achieve a similar outcome with a sophisticated and computationally expensive sampling scheme over the buffer. \newline
%Indeed, the theoretical analysis in \cite{agarwal2021online} shows that \namelo~removes bias in Q-learning type algorithms, albeit in a different sense. 
\textbf{Causality:} MDPs have a natural causal structure: actions and events in the past influence the events in the future. Therefore, whenever we see a surprising or unexpected event, we can understand why or how it happened by looking into the past. Further theoretical work is needed to realize \namel~better.

We further illustrate the same by referring to the straightforward didactic example (Section~\ref{sec:toy_example}), where we can see the effects of each of the experience replay methods. We also demonstrate superior performance on more complicated environments (Section~\ref{results}), showcasing the robustness of our approach with minimal hyperparameter tuning.

